CANUCS: An Updated Mass and Magnification Model of Abell 370 with JWST

We report an updated mass and magnification model of galaxy cluster Abell 370 using new NIRCam and NIRISS data from the CAnadian NIRISS Unbiased Cluster Survey (CANUCS). Using Lenstool and a combination of archival HST and MUSE data with new JWST data as constraints, we derive an improved gravitational lensing model and extract magnifications of background galaxies with uncertainties. Using our best fit model, we perform a search for new multiply imaged systems via predicted positions. We report no new multiply imaged systems with identifiable redshifts, likely due to already very deep HST and Spitzer data, but confirm a $z\sim8$ multiply imaged system by measuring its redshift with NIRISS and NIRSpec spectra. We find that the overall shape of the critical curve for a source at $z = 9.0$ is similar to previous models of Abell 370, with small changes. We investigate the $z\sim8$ galaxy with two images observable with an apparent magnitude in the F125W band of $26.0\pm0.2$ and $25.6\pm0.1$. After correcting for the magnifications of the images, 7.2$^{+0.2}_{-1.2}$ and 8.7$^{+0.4}_{-0.4}$, we use SED fitting to find an intrinsic stellar mass of log($M^*/M_{\odot})$ = 7.35$^{+0.04}_{-0.05}$, intrinsic SFR of 3.5$^{+2.2}_{-1.4}$ M$_{\odot}$/yr, and $M_{UV}$ of -21.3$^{+0.2}_{-0.2}$, which is close to the knee of the luminosity function at that redshift. Our model, and corresponding magnification, shear, and convergence maps are available on request and will be made publicly available on MAST in a CANUCS data release (DOI: 10.17909/ph4n-6n76).

==> multfile_rms.tex <==
\begin{table}
\begin{tabular}{cccccc}
ID & RA & Dec & z & rms(") & Catalogue \\
1.1 & 39.97629 & -1.576023 & 0.8041 & 0.31 & Gold \\
1.2 & 39.967161 & -1.576876 & 0.8041 & 0.52 & Gold \\
1.3 & 39.968546 & -1.576618 & 0.8041 & 0.17 & Gold \\
2a.1 & 39.973789 & -1.584241 & 0.7251 & 0.79 & Gold \\
2a.2 & 39.970973 & -1.585035 & 0.7251 & 0.25 & Gold \\
2a.3 & 39.968741 & -1.584507 & 0.7251 & 1.03 & Gold \\
2a.4 & 39.96956 & -1.584804 & 0.7251 & 4.93 & Gold \\
3a.1 & 39.9685154 & -1.5658046 & 1.9553 & 2.33 & Gold \\
3a.2 & 39.965677 & -1.5668566 & 1.9553 & 0.0 & Gold \\
3a.3 & 39.9789537 & -1.5674604 & 1.9553 & 0.13 & Gold \\
3b.1 & 39.9673222 & -1.5661306 & 1.9553 & 0.52 & Gold \\
3b.2 & 39.9661958 & -1.5665973 & 1.9553 & 1.52 & Gold \\
3b.3 & 39.9790446 & -1.567469 & 1.9553 & 0.21 & Gold \\
4a.1 & 39.9796721 & -1.5763896 & 1.2728 & 0.49 & Gold \\
4a.2 & 39.9707234 & -1.5762784 & 1.2728 & 0.89 & Gold \\
4a.3 & 39.9619525 & -1.5779415 & 1.2728 & 0.43 & Gold \\
4b.1 & 39.9797684 & -1.5765674 & 1.2728 & 0.52 & Gold \\
4b.2 & 39.9706752 & -1.5764562 & 1.2728 & 0.82 & Gold \\
4b.3 & 39.9620043 & -1.5780896 & 1.2728 & 0.39 & Gold \\
5.1 & 39.973486 & -1.58905 & 1.2775 & 0.11 & Gold \\
5.2 & 39.971018 & -1.589217 & 1.2775 & 1.51 & Gold \\
5.3 & 39.96913 & -1.589053 & 1.2775 & 1.9 & Gold \\
6a.1 & 39.9797577 & -1.5772207 & 1.0633 & 0.25 & Gold \\
6a.2 & 39.9693676 & -1.577354 & 1.0633 & 0.13 & Gold \\
6a.3 & 39.9644985 & -1.5783614 & 1.0633 & 0.39 & Gold \\
6b.1 & 39.9796515 & -1.5770878 & 1.0633 & 0.33 & Gold \\
6b.2 & 39.969486 & -1.5771825 & 1.0633 & 0.23 & Gold \\
6b.3 & 39.9643411 & -1.5782225 & 1.0633 & 0.37 & Gold \\
7.1 & 39.9698256 & -1.580573 & 2.7512 & 5.12 & Gold \\
7.3 & 39.968808 & -1.5856333 & 2.7512 & ----- & Bronze \\
7.4 & 39.986554 & -1.5775806 & 2.7512 & ----- & Bronze \\
7.5 & 39.961542 & -1.5800056 & 2.7512 & ----- & Bronze \\
7.6 & 39.9683489 & -1.5713448 & 2.7512 & 0.55 & Gold \\
8.1 & 39.9645508 & -1.5697533 & 1.0 & ----- & Silver \\
8.2 & 39.961868 & -1.5736833 & 1.0 & ----- & Silver \\
9.1 & 39.9624 & -1.5778861 & 1.5182 & 0.62 & Gold \\
9.2 & 39.969483 & -1.5762667 & 1.5182 & 0.72 & Gold \\
9.3 & 39.982017 & -1.5765333 & 1.5182 & 0.1 & Gold \\
11.1 & 39.963804 & -1.5693611 & 7.84 & 0.41 & Gold \\
11.2 & 39.960771 & -1.5741472 & 7.84 & 0.62 & Gold \\
12b.1 & 39.9840783 & -1.5709608 & 3.4809 & 1.49 & Gold \\
12b.2 & 39.9697827 & -1.5666566 & 3.4809 & 0.5 & Gold \\
12b.3 & 39.9591524 & -1.5754052 & 3.4809 & 0.91 & Gold \\
13.1 & 39.979532 & -1.5717869 & 4.248 & 0.74 & Gold \\
13.2 & 39.9752263 & -1.5688311 & 4.248 & 2.21 & Gold \\
13.3 & 39.9567692 & -1.5775058 & 4.248 & 0.69 & Gold \\
14a.1 & 39.9813269 & -1.5781642 & 3.1309 & 0.85 & Gold \\
14a.2 & 39.9722981 & -1.5780015 & 3.1309 & 2.54 & Gold \\
14a.3 & 39.9721943 & -1.5800387 & 3.1309 & 0.0 & Gold \\
14a.4 & 39.9576976 & -1.5804348 & 3.1309 & 0.43 & Gold \\
14a.5 & 39.9742092 & -1.5856151 & 3.1309 & 0.51 & Gold \\
14b.1 & 39.9812899 & -1.578279 & 3.1309 & ----- & Silver \\
14b.2 & 39.9723129 & -1.5782385 & 3.1309 & ----- & Silver \\
14b.4 & 39.957679 & -1.5805015 & 3.1309 & ----- & Silver \\
14b.5 & 39.9743259 & -1.5855799 & 3.1309 & ----- & Silver \\
15.1 & 39.971328 & -1.580604 & 3.7085 & ----- & Bronze \\
15.2 & 39.971935 & -1.5870512 & 3.7085 & ----- & Bronze \\
15.3 & 39.971027 & -1.5777907 & 3.7085 & ----- & Bronze \\
15.4 & 39.984017 & -1.5784514 & 3.7085 & ----- & Bronze \\
16.1 & 39.964016 & -1.5880782 & 3.7743 & ----- & Silver \\
16.2 & 39.966037 & -1.5890355 & 3.7743 & ----- & Bronze \\
16.3 & 39.984414 & -1.5841111 & 3.7743 & ----- & Silver \\
17.1 & 39.969758 & -1.5885333 & 4.2567 & 0.58 & Gold \\
17.2 & 39.985403 & -1.5808406 & 4.2567 & 0.48 & Gold \\
17.3 & 39.960235 & -1.5836508 & 4.2567 & 0.16 & Gold \\
18.1 & 39.97583 & -1.5870613 & 4.4296 & 0.25 & Gold \\
18.2 & 39.981476 & -1.5820728 & 4.4296 & 0.44 & Gold \\
18.3 & 39.957362 & -1.5820861 & 4.4296 & ----- & Silver \\
19.1 & 39.971996 & -1.5878654 & 5.6493 & ----- & Silver \\
19.2 & 39.985142 & -1.5790944 & 5.6493 & ----- & Silver \\
19.3 & 39.958316 & -1.5813093 & 5.6493 & ----- & Silver \\
20.1 & 39.965271 & -1.5878028 & 5.7505 & 1.41 & Gold \\
20.2 & 39.963608 & -1.5868833 & 5.7505 & 0.99 & Gold \\
21.1 & 39.966575 & -1.5846139 & 1.2567 & ----- & Bronze \\
21.2 & 39.967383 & -1.5850278 & 1.2567 & ----- & Bronze \\
21.3 & 39.981539 & -1.5814028 & 1.2567 & ----- & Bronze \\
22a.1 & 39.9816997 & -1.5796877 & 3.1309 & 0.28 & Gold \\
22a.2 & 39.9744221 & -1.5861106 & 3.1309 & 0.18 & Gold \\
22.3 & 39.957906 & -1.5810108 & 3.1277 & ----- & Bronze \\
23.1 & 39.980254 & -1.5667639 & 5.9386 & ----- & Silver \\
23.2 & 39.957314 & -1.572744 & 5.9386 & ----- & Silver \\
23.3 & 39.977165 & -1.5662748 & 5.9386 & ----- & Silver \\
24a.1 & 39.9635133 & -1.5702107 & 4.9153 & 0.11 & Gold \\
24a.2 & 39.9615735 & -1.5734148 & 4.9153 & 0.21 & Gold \\
24c.1 & 39.9632836 & -1.5703459 & 4.9153 & 0.31 & Gold \\
24c.2 & 39.9617365 & -1.572911 & 4.9153 & 0.47 & Gold \\
24d.1 & 39.963114 & -1.5706099 & 4.9153 & 1.0 & Gold \\
24d.2 & 39.9620561 & -1.5723396 & 4.9153 & 1.56 & Gold \\
25.1 & 39.9873002 & -1.5787754 & 3.8145 & ----- & Bronze \\
25.2 & 39.9617448 & -1.5829204 & 3.8145 & ----- & Bronze \\
25.3 & 39.966984 & -1.5867999 & 3.8084 & ----- & Bronze \\
26.1 & 39.979939 & -1.5713902 & 3.9359 & 0.27 & Gold \\
26.2 & 39.974464 & -1.5680938 & 3.9359 & 0.52 & Gold \\
26.3 & 39.957165 & -1.5769585 & 3.9359 & ----- & Silver \\
27.1 & 39.972446 & -1.567157 & 3.0161 & 0.84 & Gold \\
27.2 & 39.980694 & -1.571125 & 3.0161 & 0.71 & Gold \\
27.3 & 39.95829 & -1.5759068 & 3.0161 & 0.62 & Gold \\
28.1 & 39.963492 & -1.5822806 & 2.9101 & 0.32 & Gold \\
28.2 & 39.967058 & -1.5845583 & 2.9101 & 0.24 & Gold \\
28.3 & 39.987816 & -1.5774528 & 2.9101 & ----- & Silver \\
29a.1 & 39.9834878 & -1.5673115 & 4.4897 & 1.36 & Gold \\
29a.2 & 39.9684473 & -1.5646408 & 4.4897 & 0.92 & Gold \\
29a.3 & 39.9601989 & -1.5694708 & 4.4897 & 1.59 & Gold \\
29b.1 & 39.9835804 & -1.5675745 & 4.4897 & 0.21 & Gold \\
29b.2 & 39.9676432 & -1.5649075 & 4.4897 & 0.68 & Gold \\
29b.3 & 39.9609326 & -1.5690004 & 4.4897 & 0.63 & Gold \\
30.1 & 39.983351 & -1.5704081 & 5.6459 & ----- & Silver \\
30.2 & 39.972404 & -1.5663533 & 5.6459 & ----- & Silver \\
31.1 & 39.972404 & -1.5693301 & 5.4476 & ----- & Bronze \\
31.2 & 39.980667 & -1.5747346 & 5.4476 & ----- & Bronze \\
31.3 & 39.956158 & -1.5786786 & 5.4476 & ----- & Bronze \\
32.1 & 39.966286 & -1.5693446 & 4.4953 & ----- & Bronze \\
32.2 & 39.988098 & -1.5751871 & 4.4953 & ----- & Bronze \\
32.3 & 39.960682 & -1.5783795 & 4.4953 & ----- & Bronze \\
33.1 & 39.962723 & -1.5860035 & 4.882 & ----- & Bronze \\
33.2 & 39.966217 & -1.5879961 & 4.882 & ----- & Bronze \\
34.1 & 39.970108 & -1.5701499 & 5.2437 & ----- & Bronze \\
34.2 & 39.971806 & -1.5880395 & 5.2437 & ----- & Bronze \\
34.3 & 39.958565 & -1.5817008 & 5.2437 & ----- & Bronze \\
34.4 & 39.985046 & -1.579559 & 5.2437 & ----- & Bronze \\
35.1 & 39.981541 & -1.5658624 & 6.1735 & ----- & Bronze \\
35.2 & 39.975826 & -1.5644423 & 6.1735 & ----- & Bronze \\
36.1 & 39.962444 & -1.5807098 & 6.2855 & ----- & Bronze \\
36.2 & 39.965996 & -1.5843844 & 6.2855 & ----- & Bronze \\
37.1 & 39.97039 & -1.5687943 & 5.6489 & ----- & Bronze \\
37.2 & 39.970428 & -1.5694203 & 5.6489 & ----- & Bronze \\
38.1 & 39.9771985 & -1.5738047 & 3.2 & 0.77 & Gold \\
38.2 & 39.9750827 & -1.5721194 & 3.2 & 2.27 & Gold \\
39.1 & 39.965442 & -1.5780222 & 1.2777 & ----- & Bronze \\
39.2 & 39.967933 & -1.5773472 & 1.2777 & ----- & Bronze \\
39.3 & 39.982296 & -1.576975 & 1.2777 & ----- & Bronze \\
40.1 & 39.963579 & -1.5656333 & 1.0323 & ----- & Bronze \\
40.2 & 39.962958 & -1.5661111 & 1.0323 & ----- & Bronze \\
40.3 & 39.963375 & -1.5659528 & 1.0323 & ----- & Bronze \\
41.1 & 39.970546 & -1.5693801 & 4.9441 & ----- & Bronze \\
41.2 & 39.969977 & -1.5700367 & 4.9441 & ----- & Bronze \\
41.3 & 39.985223 & -1.5793885 & 4.9441 & ----- & Bronze \\
41.4 & 39.971395 & -1.58802 & 4.9441 & ----- & Bronze \\
42.1 & 39.970632 & -1.5710393 & 4.3381 & ----- & Bronze \\
42.2 & 39.983162 & -1.5796664 & 4.3381 & ----- & Bronze \\
42.3 & 39.973383 & -1.5874465 & 4.3381 & ----- & Bronze \\
42.4 & 39.957967 & -1.5815081 & 4.3381 & ----- & Bronze \\
\end{tabular}
\end{table}


==> multfile_withrms.tex <==
\begin{table}
\begin{tabular}{cccccc}
ID & RA & Dec & z & rms(") & Catalogue \\
1a.1 & 39.9762942 & -1.5760362 & 0.8041 & 0.673 & Gold \\
1a.2 & 39.9671518 & -1.576882 & 0.8041 & 0.471 & Gold \\
1a.3 & 39.9685746 & -1.5766236 & 0.8041 & 0.230 & Gold \\
1b.2 & 39.9675631 & -1.5767597 & 0.8041 & 0.06 & Gold \\
1b.3 & 39.9680966 & -1.5766598 & 0.8041 & 0.06 & Gold \\
1c.2 & 39.9670351 & -1.5769042 & 0.8041 & 0.207 & Gold \\
1c.3 & 39.9687358 & -1.5765875 & 0.8041 & 0.207 & Gold \\
2a.1 & 39.973789 & -1.584241 & 0.7251 & 0.496 & Gold \\
2a.2 & 39.970973 & -1.585035 & 0.7251 & 0.207 & Gold \\
2a.3 & 39.968741 & -1.584507 & 0.7251 & 0.557 & Gold \\
3a.1 & 39.9685154 & -1.5658046 & 1.9553 & 0.573 & Gold \\
3a.2 & 39.965677 & -1.5668566 & 1.9553 & 0.331 & Gold \\
3a.3 & 39.9789537 & -1.5674604 & 1.9553 & 0.543 & Gold \\
3b.1 & 39.9673222 & -1.5661306 & 1.9553 & 0.534 & Gold \\
3b.2 & 39.9661958 & -1.5665973 & 1.9553 & 0.161 & Gold \\
3b.3 & 39.9790446 & -1.567469 & 1.9553 & 0.663 & Gold \\
4a.1 & 39.9796721 & -1.5763896 & 1.2728 & 0.617 & Gold \\
4a.2 & 39.9707234 & -1.5762784 & 1.2728 & 0.547 & Gold \\
4a.3 & 39.9619525 & -1.5779415 & 1.2728 & 0.487 & Gold \\
4b.1 & 39.9797684 & -1.5765674 & 1.2728 & 0.657 & Gold \\
4b.2 & 39.9706752 & -1.5764562 & 1.2728 & 0.492 & Gold \\
4b.3 & 39.9620043 & -1.5780896 & 1.2728 & 0.457 & Gold \\
4c.1 & 39.9795892 & -1.5762564 & 1.2728 & 0.551 & Gold \\
4c.2 & 39.9707553 & -1.5761507 & 1.2728 & 0.574 & Gold \\
4c.3 & 39.9619075 & -1.5778271 & 1.2728 & 0.535 & Gold \\
5.1 & 39.973486 & -1.58905 & 1.2775 & 0.478 & Gold \\
5.2 & 39.971018 & -1.589217 & 1.2775 & 0.263 & Gold \\
5.3 & 39.96913 & -1.589053 & 1.2775 & 0.368 & Gold \\
6a.1 & 39.9797577 & -1.5772207 & 1.0633 & 0.252 & Gold \\
6a.2 & 39.9693676 & -1.577354 & 1.0633 & 0.155 & Gold \\
6a.3 & 39.9644985 & -1.5783614 & 1.0633 & 0.348 & Gold \\
6b.1 & 39.9796515 & -1.5770878 & 1.0633 & 0.372 & Gold \\
6b.2 & 39.969486 & -1.5771825 & 1.0633 & 0.15 & Gold \\
6b.3 & 39.9643411 & -1.5782225 & 1.0633 & 0.343 & Gold \\
6c.1 & 39.9794544 & -1.5770341 & 1.0633 & 0.367 & Gold \\
6c.2 & 39.969659 & -1.5770966 & 1.0633 & 0.182 & Gold \\
6c.3 & 39.9640847 & -1.5781854 & 1.0633 & 0.428 & Gold \\
7.1 & 39.9698256 & -1.580573 & 2.7512 & 0.638 & Gold \\
7.3 & 39.968808 & -1.5856333 & 2.7512 & ----- & Silver \\
7.4 & 39.986554 & -1.5775806 & 2.7512 & ----- & Silver \\
7.5 & 39.961542 & -1.5800056 & 2.7512 & ----- & Silver \\
7.6 & 39.9683489 & -1.5713448 & 2.7512 & 0.638 & Gold \\
8.1 & 39.9645508 & -1.5697533 & 2.8659 & 0.06 & Gold \\
8.2 & 39.961868 & -1.5736833 & 2.8659 & 0.06 & Gold \\
9.1 & 39.9624 & -1.5778861 & 1.5182 & 0.662 & Gold \\
9.2 & 39.969483 & -1.5762667 & 1.5182 & 0.629 & Gold \\
9.3 & 39.982017 & -1.5765333 & 1.5182 & 0.15 & Gold \\
11a.1 & 39.9637986 & -1.5693826 & 7.6476 & 0.099 & Gold \\
11a.2 & 39.960764 & -1.5741493 & 7.6476 & 0.099 & Gold \\
11b.1 & 39.9638653 & -1.569316 & 7.6476 & 0.127 & Gold \\
11b.2 & 39.9607279 & -1.5742159 & 7.6476 & 0.127 & Gold \\
12a.1 & 39.9841376 & -1.5708867 & 3.4809 & 0.736 & Gold \\
12a.2 & 39.9696122 & -1.5666344 & 3.4809 & 0.302 & Gold \\
12a.3 & 39.9592413 & -1.5752348 & 3.4809 & 0.552 & Gold \\
12b.1 & 39.9840783 & -1.5709608 & 3.4809 & 0.755 & Gold \\
12b.2 & 39.9697827 & -1.5666566 & 3.4809 & 0.236 & Gold \\
12b.3 & 39.9591524 & -1.5754052 & 3.4809 & 0.620 & Gold \\
12c.1 & 39.9839791 & -1.5707975 & 3.4809 & 0.672 & Gold \\
12c.2 & 39.9698687 & -1.5665785 & 3.4809 & 0.292 & Gold \\
12c.3 & 39.9591413 & -1.5752015 & 3.4809 & 0.501 & Gold \\
13a.1 & 39.9795197 & -1.5717758 & 4.248 & 0.616 & Gold \\
13a.2 & 39.9752181 & -1.5688202 & 4.248 & 0.947 & Gold \\
13a.3 & 39.9567562 & -1.5774992 & 4.248 & 1.426 & Gold \\
13b.1 & 39.9795809 & -1.5718161 & 4.248 & 0.544 & Gold \\
13b.2 & 39.9751362 & -1.5687702 & 4.248 & 0.544 & Gold \\
14a.1 & 39.9813269 & -1.5781642 & 3.1309 & 0.489 & Gold \\
14a.2 & 39.9722981 & -1.5780015 & 3.1309 & 0.771 & Gold \\
14a.3 & 39.9721943 & -1.5800387 & 3.1309 & 1.384 & Gold \\
14a.4 & 39.9576976 & -1.5804348 & 3.1309 & 0.401 & Gold \\
14a.5 & 39.9742092 & -1.5856151 & 3.1309 & 0.638 & Gold \\
14b.1 & 39.9812899 & -1.578279 & 3.1309 & 0.207 & Gold \\
14b.2 & 39.9723129 & -1.5782385 & 3.1309 & 0.461 & Gold \\
14b.4 & 39.957679 & -1.5805015 & 3.1309 & 0.772 & Gold \\
14b.5 & 39.9743259 & -1.5855799 & 3.1309 & 0.289 & Gold \\
15.1 & 39.971328 & -1.580604 & 3.7085 & ----- & Bronze \\
15.2 & 39.971935 & -1.5870512 & 3.7085 & ----- & Bronze \\
15.3 & 39.971027 & -1.5777907 & 3.7085 & ----- & Bronze \\
15.4 & 39.984017 & -1.5784514 & 3.7085 & ----- & Bronze \\
16.1 & 39.964016 & -1.5880782 & 3.7743 & ----- & Silver \\
16.2 & 39.966037 & -1.5890355 & 3.7743 & ----- & Bronze \\
16.3 & 39.984414 & -1.5841111 & 3.7743 & ----- & Silver \\
17.1 & 39.969758 & -1.5885333 & 4.2567 & 0.446 & Gold \\
17.2 & 39.985403 & -1.5808406 & 4.2567 & 0.562 & Gold \\
17.3 & 39.960235 & -1.5836508 & 4.2567 & 0.366 & Gold \\
18.1 & 39.97583 & -1.5870613 & 4.4296 & 0.234 & Gold \\
18.2 & 39.981476 & -1.5820728 & 4.4296 & 0.234 & Gold \\
19.1 & 39.971996 & -1.5878654 & 5.6493 & ----- & Silver \\
19.2 & 39.985142 & -1.5790944 & 5.6493 & ----- & Silver \\
19.3 & 39.958316 & -1.5813093 & 5.6493 & ----- & Silver \\
20.1 & 39.965271 & -1.5878028 & 5.7505 & 0.555 & Gold \\
20.2 & 39.963608 & -1.5868833 & 5.7505 & 0.555 & Gold \\
21.1 & 39.966575 & -1.5846139 & 1.2567 & ----- & Bronze \\
21.2 & 39.967383 & -1.5850278 & 1.2567 & ----- & Bronze \\
21.3 & 39.981539 & -1.5814028 & 1.2567 & ----- & Bronze \\
22a.1 & 39.981683 & -1.5796827 & 3.1309 & 0.328 & Gold \\
22a.2 & 39.9744122 & -1.5861063 & 3.1309 & 0.328 & Gold \\
22b.1 & 39.9816163 & -1.5798189 & 3.1309 & 0.307 & Gold \\
22b.2 & 39.9745178 & -1.5860563 & 3.1309 & 0.307 & Gold \\
23.1 & 39.980254 & -1.5667639 & 5.9386 & ----- & Silver \\
23.2 & 39.957314 & -1.572744 & 5.9386 & ----- & Silver \\
23.3 & 39.977165 & -1.5662748 & 5.9386 & ----- & Silver \\
24a.1 & 39.9635133 & -1.5702107 & 4.9153 & 0.051 & Gold \\
24a.2 & 39.9615735 & -1.5734148 & 4.9153 & 0.051 & Gold \\
24b.1 & 39.9634818 & -1.5702422 & 4.9153 & 0.051 & Gold \\
24b.2 & 39.9615957 & -1.573374 & 4.9153 & 0.051 & Gold \\
24c.1 & 39.9632836 & -1.5703459 & 4.9153 & 0.067 & Gold \\
24c.2 & 39.9617365 & -1.572911 & 4.9153 & 0.067 & Gold \\
24d.1 & 39.963114 & -1.5706099 & 4.9153 & 0.268 & Gold \\
24d.2 & 39.9620561 & -1.5723396 & 4.9153 & 0.268 & Gold \\
24e.1 & 39.9630029 & -1.5706265 & 4.916 & 0.249 & Gold \\
24e.2 & 39.9621432 & -1.5719822 & 4.916 & 0.249 & Gold \\
24f.1 & 39.9630844 & -1.570708 & 4.916 & 0.352 & Gold \\
24f.2 & 39.9622377 & -1.5720674 & 4.916 & 0.352 & Gold \\
25a.1 & 39.9872963 & -1.5787605 & 3.8145 & 0.099 & Gold \\
25a.2 & 39.9617351 & -1.5828757 & 3.8145 & 0.099 & Gold \\
25b.1 & 39.9872393 & -1.5789939 & 3.8145 & 0.137 & Gold \\
25b.2 & 39.9619074 & -1.5832451 & 3.8145 & 0.137 & Gold \\
25c.1 & 39.987274 & -1.5788161 & 3.8145 & 0.103 & Gold \\
25c.2 & 39.9617546 & -1.5829368 & 3.8145 & 0.103 & Gold \\
26.1 & 39.979939 & -1.5713902 & 3.9359 & 0.541 & Gold \\
26.2 & 39.974464 & -1.5680938 & 3.9359 & 0.541 & Gold \\
26.3 & 39.957165 & -1.5769585 & 3.9359 & ----- & Silver \\
27.1 & 39.972446 & -1.567157 & 3.0161 & 0.492 & Gold \\
27.2 & 39.980694 & -1.571125 & 3.0161 & 0.372 & Gold \\
27.3 & 39.95829 & -1.5759068 & 3.0161 & 0.15 & Gold \\
28.1 & 39.963492 & -1.5822806 & 2.9101 & 0.665 & Gold \\
28.2 & 39.967058 & -1.5845583 & 2.9101 & 0.665 & Gold \\
28.3 & 39.987816 & -1.5774528 & 2.9101 & ----- & Silver \\
29a.1 & 39.9834878 & -1.5673115 & 4.4897 & 0.487 & Gold \\
29a.2 & 39.9684473 & -1.5646408 & 4.4897 & 0.476 & Gold \\
29a.3 & 39.9601989 & -1.5694708 & 4.4897 & 0.837 & Gold \\
29b.1 & 39.9835804 & -1.5675745 & 4.4897 & 0.991 & Gold \\
29b.2 & 39.9676432 & -1.5649075 & 4.4897 & 0.079 & Gold \\
29b.3 & 39.9609326 & -1.5690004 & 4.4897 & 0.952 & Gold \\
30.1 & 39.983351 & -1.5704081 & 5.6459 & ----- & Silver \\
30.2 & 39.972404 & -1.5663533 & 5.6459 & ----- & Silver \\
31.1 & 39.972404 & -1.5693301 & 5.4476 & ----- & Bronze \\
31.2 & 39.980667 & -1.5747346 & 5.4476 & ----- & Bronze \\
31.3 & 39.956158 & -1.5786786 & 5.4476 & ----- & Bronze \\
32.1 & 39.966286 & -1.5693446 & 4.4953 & ----- & Bronze \\
32.2 & 39.988098 & -1.5751871 & 4.4953 & ----- & Bronze \\
32.3 & 39.960682 & -1.5783795 & 4.4953 & ----- & Bronze \\
33.1 & 39.962723 & -1.5860035 & 4.882 & ----- & Bronze \\
33.2 & 39.966217 & -1.5879961 & 4.882 & ----- & Bronze \\
34.1 & 39.970108 & -1.5701499 & 5.2437 & ----- & Bronze \\
34.2 & 39.971806 & -1.5880395 & 5.2437 & ----- & Bronze \\
34.3 & 39.958565 & -1.5817008 & 5.2437 & ----- & Bronze \\
34.4 & 39.985046 & -1.579559 & 5.2437 & ----- & Bronze \\
35.1 & 39.981541 & -1.5658624 & 6.1735 & ----- & Bronze \\
35.2 & 39.975826 & -1.5644423 & 6.1735 & ----- & Bronze \\
36.1 & 39.962444 & -1.5807098 & 6.2855 & ----- & Bronze \\
36.2 & 39.965996 & -1.5843844 & 6.2855 & ----- & Bronze \\
37.1 & 39.97039 & -1.5687943 & 5.6489 & ----- & Bronze \\
37.2 & 39.970428 & -1.5694203 & 5.6489 & ----- & Bronze \\
38.1 & 39.9771985 & -1.5738047 & 3.2 & 0.684 & Gold \\
38.2 & 39.9750827 & -1.5721194 & 3.2 & 0.684 & Gold \\
39.1 & 39.965442 & -1.5780222 & 1.2777 & ----- & Bronze \\
39.2 & 39.967933 & -1.5773472 & 1.2777 & ----- & Bronze \\
39.3 & 39.982296 & -1.576975 & 1.2777 & ----- & Bronze \\
40.1 & 39.963579 & -1.5656333 & 1.0323 & ----- & Bronze \\
40.2 & 39.962958 & -1.5661111 & 1.0323 & ----- & Bronze \\
40.3 & 39.963375 & -1.5659528 & 1.0323 & ----- & Bronze \\
41.1 & 39.970546 & -1.5693801 & 4.9441 & ----- & Bronze \\
41.2 & 39.969977 & -1.5700367 & 4.9441 & ----- & Bronze \\
41.3 & 39.985223 & -1.5793885 & 4.9441 & ----- & Bronze \\
41.4 & 39.971395 & -1.58802 & 4.9441 & ----- & Bronze \\
42.1 & 39.970632 & -1.5710393 & 4.3381 & ----- & Bronze \\
42.2 & 39.983162 & -1.5796664 & 4.3381 & ----- & Bronze \\
42.3 & 39.973383 & -1.5874465 & 4.3381 & ----- & Bronze \\
42.4 & 39.957967 & -1.5815081 & 4.3381 & ----- & Bronze \\
43.1 & 39.9824 & -1.5811 & 8.197 & ----- & Silver \\
43.2 & 39.975875 & -1.58726 & 8.197 & ----- & Silver \\
\end{tabular}
\end{table}

